HTS: A Hardware Task Scheduler for Heterogeneous Systems

As the Moore's scaling era comes to an end, application specific hardware accelerators appear as an attractive way to improve the performance and power efficiency of our computing systems. A massively heterogeneous system with a large number of hardware accelerators along with multiple general purpose CPUs is a promising direction, but pose several challenges in terms of the run-time scheduling of tasks on the accelerators and design granularity of accelerators. This paper addresses these challenges by developing an example heterogeneous system to enable multiple applications to share the available accelerators. We propose to design accelerators at a lower abstraction to enable applications to be broken down into tasks that can be mapped on several accelerators. We observe that several real-life workloads can be broken down into common primitives that are shared across many workloads. Finally, we propose and design a hardware task scheduler inspired by the hardware schedulers in out-of-order superscalar processors to efficiently utilize the accelerators in the system by scheduling tasks in out-of-order and even speculatively. We evaluate the proposed system on both real-life and synthetic benchmarks based on Digital Signal Processing~(DSP) applications. Compared to executing the benchmark on a system with sequential scheduling, proposed scheduler achieves up to 12x improvement in performance.

==> simulation.tex <==
\section{Simulation Environment}
\label{sec:sim}
% why do we need a simulation environment ?
The development of heterogeneous systems with specialized accelerators is in early stages. So, it is difficult to get access to a fully-functional large-scale computing system apart from System-On-Chip (SoC) setups. We do not intend to experiment with SoCs since we are proposing a server-level system whose design goals may not coincide with mobile platform system, for instance - mobile SoCs are built to run low power mobile devices, which may not be a strict requirement for a more general system. Also, we intend to encounter many system-level design issues like accelerator resource management and arbitration, rapid accelerator design space exploration, communication between accelerators, and how CPUs and memory hierarchy impact accelerator performance~\cite{parade}. Thus, we look for a full-system research simulation platform which enables us to perform complete design space exploration and analysis. 

% categories of simulation environment
Cong et.al ~\cite{parade} present four main categories for such research platforms : 
\begin{enumerate}
\item {Virtual Prototyping platform - It aides in fast modelling of traditional multi-processor SoC (MPSoC) architectures. It is difficult to model systems with a sea of accelerators with such platforms as they are limited to SoC design. They are inefficient in handling complex network-on-chips, complex cache memory hierarchies etc. Examples are ~\cite{trimedia} and ~\cite{synopsys}. 
}
\item{
FPGA Prototyping platform - It utilizes existing field programmable SoC and implements accelerators in FPGA. It is constrained by tedious FPGA implementation efforts and resources. Examples are ~\cite{linqits} and ~\cite{memcached}.
}
\item{
RTL Simulation - It is also constrained by tedious implementation efforts. Examples are ~\cite{accstore} and ~\cite{sonic}.
}
\item{
Flexible cycle-accurate full-system Simulation - It mimics real life system, but number of complete platforms is limited as it takes multiple person-year efforts~\cite{transformer}. Examples are ~\cite{domainspecacc} and ~\cite{charmcong}.
}
\end{enumerate}
We choose fourth category as it allows us to explore system-level design issues. We pick two prominent simulation environments for further analysis.

% Aladdin - one paragraph
\subsection{Gem5-Aladdin}
It integrates standalone accelerator simulator Aladdin~\cite{aladdin} and full-system simulator gem5~\cite{gem5}, and enables modelling interactions between accelerators and CPUs, hardware-managed caches, DMA and virtual memory. It has two modes of simulation - syscall emulation and full-system simulation, where the latter allows one to incorporate operating system phenomenons like device driver to hardware interactions.

Aladdin models power, performance and cycle-level activity of fixed function accelerators without generating RTL. It constructs a dynamic data dependence graph as a dataflow representation of a accelerator by profiling dynamic execution of a program, where the graph vertices are LLVM IR instructions and edges are true dependencies between them. After applying common design optimisations and user-defines hardware constraints, it performs a breadth first traversal to schedule graph for execution.

It allows accelerators to leverage DMA engine present in gem5. To do so, programmer can insert calls to \textit{dmaLoad} and \textit{dmaStore} within the accelerated funtion accompanied with its parameters.

It affords the availability of caches to individual accelerators. It uses gem5's cache model attached with MOESI cache coherence protocol. It also supports virtual memory through custom-made Aladdin TLB model~\cite{gem5aladdin}. Shao et.al cite two reasons for not using gem5's existing TLB models - 1) Resident TLB models are tied to particular ISAs and 2) the trace address Aladdin uses does not directly map to the simulated address space that CPU is accessing. Their model translates trace address to a simulated virtual address and then to a simulated physical address, where TLB misses are modelled with pre-characterised miss penalty~\cite{gem5aladdin}.

To invoke an accelerator, a user program should make a \textit{ioctl} system call, where each accelerator is assigned a command number. The CPU can either spin wait or continue with program execution periodically checking the status variable. After completing its compute, the accelerator writes to pointer location shared with the CPU, and CPU notices the update due to presence of coherence in the system. Note that the accelerator issues an \textit{mfence} before signaling the CPU to resolve memory consistency issues.

% Parade - one paragraph
\subsection{PARADE}
Platform for Accelerator-Rich Architectural Design and Exploration (PARADE)~\cite{parade} is a cycle-accurate full-system simulation environment. It models each accelerator using high-level synthesis tools, and provides a workflow to automatically generate dedicated/composable accelerator modules for integration. Notably, it provides a cycle-accurate model of a central hardware to manage entire system, eloquently termed as Global Accelerator Manager (GAM), similar in terms of higher level functionality to what we propose. Also, it uses cycle-accurate full-system simulator gem5~\cite{gem5} to model coherent cache/scratchpad with shared memory between CPU cores and accelerators etc.

Both the environments satisfy our higher level requirements, each bearing its advantages and disadvantages. PARADE is complete with the presence of a central task manager, but it only models traditional DMA-based accelerators where all data must be copied to local scratchpads before compute begins, which imposes a constraint on the input size of a compute. In contrast, gem5-aladdin is able to model a cache-based accelerator which can give variable latency memory accesses and optimisations on DMA, though it does not support full-system simulation in practice as mentioned in ~\cite{gem5aladdingit}.

==> status.tex <==
\appendix

This section is a supplementary material intended to provide status of the project as of March 27th 2018. \\

What all have we done?
\begin{enumerate}
\item Observing the advent of many specialized accelerators, we envisioned a modern day computing system and formalized its proposal.  
\item We performed an elaborate literature survey on task-based programming models and architectures, specifically looking for hardware task scheduler based systems. 
\item We probed recent literature to filter out simulation environments and performed specific case studies to select one of them. We spent time deliberating on the toy application domain to be chosen for illustration. 
\item We have coded up the requisite accelerators for our toy application domain using gem5-Aladdin to get accurate cycle, power and area values. 
\item We completed the design of an out-of-order based design for our hardware task scheduler
\end{enumerate}

What do we plan to achieve?
\begin{enumerate}
\item Next, we intend to implement our design of hardware task scheduler and interface it with our system consisting of sea of accelerators. We intend to spawn different applications using our kernels and validate the employment of such a system by performing an in-depth analysis. 
\item we will effectively show that we can get speed-ups by breaking applications into tasks and accelerating them on multiple accelerators.
\item We also intend to work on the programming model to be used for such a system, if time permits. 
\item We aim to submit the work to HPCA 2019.
\end{enumerate}
